Add force and/or change underlying projection method to improve accuracy of Explicit Robin-Neumann and fully decoupled schemes for the coupling of incompressible fluid with thin-walled structure

This work aims at providing some novel and practical ideas to improve accuracy of some partitioned algorithms, precisely Fernandez's Explicit Robin-Neumann and fully decoupled schemes, for the coupling of incompressible fluid with thin-walled structure. Inspired by viscosity of fluid and justified by boundary layer theory, the force between fluid and structure corresponding to viscosity is increased. Numerical experiments demonstrate improvement of accuracy under such modification. To improve accuracy of fully decoupled schemes further, the underlying projection method is replaced.

==> images/subfigure_example.tex <==
\begin{figure}[h]
  \centering
  \begin{subfigure}[h]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{not_applicable.png}
    \caption{rate = 2}
    \label{fig:five over x}
  \end{subfigure}
  \begin{subfigure}[h]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{rn_m1_r1_rate3_beta43.pdf}
    \caption{rate = 3}
    \label{fig:y equals x}
  \end{subfigure}

  \begin{subfigure}[h]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{rn_m1_r1_rate4_beta43.pdf}
    \caption{rate = 4}
    \label{fig:three sin x}
  \end{subfigure}
  \begin{subfigure}[h]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{rn_m1_r1_rate5_beta43.pdf}
    \caption{rate = 5}
    \label{fig:five over x}
  \end{subfigure}
  \caption{Structure displacement of Fernandez Explicit Robin-Neumann scheme (Fern ERN) and Algorithm 1 (Algo 1) with $\beta = 43$ at final time}
  \label{fig:three graphs}
\end{figure}


==> tables/nouse.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{ l l l }
\hline
rate & $ E_{rate} $  & $ O_{rate} $    \\
\hline
0 &			 0.959089  &  \\
1 &			 0.719217 &	 0.415238 \\
2 &			 0.435036 &	 0.725292 \\
3 &			 0.241714 &	 0.847834 \\
4 &			 0.128601 &	 0.910399 \\
\hline
\end{tabular}
\caption{Numerical results of explicit Robin-Neumann  scheme ("F 10 S 10" IMERN) }
\label{table:ern}
\end{table}

